Deep learning approaches to indoor wireless channel estimation for low-power communication

In the rapidly growing development of the Internet of Things (IoT) infrastructure, achieving reliable wireless communication is a challenge. IoT devices operate in diverse environments with common signal interference and fluctuating channel conditions. Accurate channel estimation helps adapt the transmission strategies to current conditions, ensuring reliable communication. Traditional methods, such as Least Squares (LS) and Minimum Mean Squared Error (MMSE) estimation techniques, often struggle to adapt to the diverse and complex environments typical of IoT networks. This research article delves into the potential of Deep Learning (DL) to enhance channel estimation, focusing on the Received Signal Strength Indicator (RSSI) metric - a critical yet challenging aspect due to its susceptibility to noise and environmental factors. This paper presents two Fully Connected Neural Networks (FCNNs)-based Low Power (LP-IoT) channel estimation models, leveraging RSSI for accurate channel estimation in LP-IoT communication. Our Model A exhibits a remarkable 99.02% reduction in Mean Squared Error (MSE), and Model B demonstrates a notable 90.03% MSE reduction compared to the benchmarks set by current studies. Additionally, the comparative studies of our model A with other DL-based techniques show significant efficiency in our estimation models.

==> Tables/Comparison-traditional-old.tex <==
\begin{table}[]
\centering
\caption{Comparison of proposed models A and B with traditional estimation techniques}
\label{tab:Comparison-Traditional}
\begin{tabular}{|lll|}
\hline
\multicolumn{3}{|c|}{\textbf{Estimation Error}}                             \\ \hline
\multicolumn{1}{|l|}{\textbf{Scenario-1}}                      & \multicolumn{1}{l|}{\textbf{MSE}}                 & \textbf{RMSE} \\ \hline
\rowcolor[HTML]{CBCEFB} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{CBCEFB}\begin{tabular}[c]{@{}c@{}}Proposed Model A\\ (Scenario-1)\end{tabular}}              \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}\textbf{Case I}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.10} & 0.32          \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}\textbf{Case II}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.23} & 0.48          \\ \hline
\rowcolor[HTML]{ECF4FF} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{ECF4FF}\textbf{Autoregression Model}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Case I}}   & \multicolumn{1}{l|}{0.10}  & 0.32 \\ \hline
\multicolumn{1}{|l|}{\textbf{Case II}}  & \multicolumn{1}{l|}{0.24}  & 0.49 \\ \hline
\rowcolor[HTML]{ECF4FF} 
\multicolumn{3}{|c|}{\cellcolor[HTML]{ECF4FF}\textbf{Moving Average Model}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Case I}}   & \multicolumn{1}{l|}{0.10}  & 0.32 \\ \hline
\multicolumn{1}{|l|}{\textbf{Case II}}  & \multicolumn{1}{l|}{0.24}  & 0.49 \\ \hline
\end{tabular}
\end{table}

==> Tables/Comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\renewcommand{\arraystretch}{1.5} % Change the 1.5 to increase or decrease spacing

\begin{table*}[t]
\centering
%\tiny
\caption{The comparative analysis of FCNN-based estimation model A with other DL-based techniques.}
\label{tab:Comparison}
\begin{tabular}{|llllllllll|}
\hline
\multicolumn{1}{|l|}{\textbf{Models}} &
  \multicolumn{2}{l|}{\textbf{Training}} &
  \multicolumn{2}{l|}{\textbf{Testing}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   \\ \cline{1-5}
\multicolumn{1}{|l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Estimation\\ Models\end{tabular}}} &
  \multicolumn{1}{l|}{\textbf{MSE}} &
  \multicolumn{1}{l|}{\textbf{RMSE}} &
  \multicolumn{1}{l|}{\textbf{MSE}} &
  \multicolumn{1}{l|}{\textbf{RMSE}} &
  \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Training \\ Time\\ (Secs)\end{tabular}}}} &
  \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Testing\\  Time\\ (Secs)\end{tabular}}}} &
  \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Training \\ Memory\\  Usage\\ (KBs)\end{tabular}}}} &
  \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Testing\\  Memory\\  Usage\\ (KBs)\end{tabular}}}} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}No. of \\ Trainable\\  Parameaers\end{tabular}}} \\ \hline
\multicolumn{10}{|c|}{\textbf{Proposed FCNN-based Model A}} \\ \hline
\rowcolor[HTML]{CBCEFB} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{CBCEFB}\textbf{Case I}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}49.38} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}7.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}0.11} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}0.34} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}0.954} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}0.006} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}675668} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}676296} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}} \\ \cline{1-9}
\rowcolor[HTML]{CBCEFB} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{CBCEFB}\textbf{Case II}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}35.93} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}5.99} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}0.23} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}0.48} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}1.792} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}0.002} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}743108} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{CBCEFB}743108} &
  \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{CBCEFB}231}} \\ \hline
\multicolumn{10}{|c|}{\textbf{Recurrent Neural Network (RNN)-based Model}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Case I}} &
  \multicolumn{1}{l|}{0.37} &
  \multicolumn{1}{l|}{0.61} &
  \multicolumn{1}{l|}{0.10} &
  \multicolumn{1}{l|}{0.32} &
  \multicolumn{1}{l|}{300.687} &
  \multicolumn{1}{l|}{0.008} &
  \multicolumn{1}{l|}{940784} &
  \multicolumn{1}{l|}{706372} &
  \multicolumn{1}{c|}{} \\ \cline{1-9}
\multicolumn{1}{|l|}{\textbf{Case II}} &
  \multicolumn{1}{l|}{0.22} &
  \multicolumn{1}{l|}{0.47} &
  \multicolumn{1}{l|}{0.24} &
  \multicolumn{1}{l|}{0.49} &
  \multicolumn{1}{l|}{314.708} &
  \multicolumn{1}{l|}{0.006} &
  \multicolumn{1}{l|}{975988} &
  \multicolumn{1}{l|}{721780} &
  \multicolumn{1}{c|}{\multirow{-2}{*}{4353}} \\ \hline
\multicolumn{10}{|c|}{\textbf{Long Short Term Memory (LSTM)-based Model}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Case I}} &
  \multicolumn{1}{l|}{0.37} &
  \multicolumn{1}{l|}{0.61} &
  \multicolumn{1}{l|}{0.11} &
  \multicolumn{1}{l|}{0.32} &
  \multicolumn{1}{l|}{292.700} &
  \multicolumn{1}{l|}{0.230} &
  \multicolumn{1}{l|}{975988} &
  \multicolumn{1}{l|}{727884} &
  \multicolumn{1}{c|}{} \\ \cline{1-9}
\multicolumn{1}{|l|}{\textbf{Case II}} &
  \multicolumn{1}{l|}{0.22} &
  \multicolumn{1}{l|}{0.47} &
  \multicolumn{1}{l|}{0.24} &
  \multicolumn{1}{l|}{0.49} &
  \multicolumn{1}{l|}{312.110} &
  \multicolumn{1}{l|}{0.160} &
  \multicolumn{1}{l|}{1021652} &
  \multicolumn{1}{l|}{742744} &
  \multicolumn{1}{c|}{\multirow{-2}{*}{26641}} \\ \hline

\end{tabular}
\end{table*}

==> Tables/Results.tex <==
% Please add the following required packages to your document preamble:

\begin{table*}[t]
\centering
\caption{Results of channel estimation by random forest algorithm.}
\label{tab:RF-Results}
\begin{tabular}{|l|ll|ll|l|l|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Random Forest\\ Algorithm for \\ Channel Estimation \\ in LP-IoT Devices\end{tabular}}} &
  \multicolumn{2}{l|}{\textbf{Training}} &
  \multicolumn{2}{l|}{\textbf{Testing}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Training\\  time (Secs)\end{tabular}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Testing\\  time (Secs)\end{tabular}}} \\ \cline{2-5}
 &
  \multicolumn{1}{l|}{\textbf{MSE}} &
  \textbf{RMSE} &
  \multicolumn{1}{l|}{\textbf{MSE}} &
  \textbf{RMSE} &
   &
   \\ \hline
\textbf{Combined Scenarios} &
  \multicolumn{1}{l|}{3.16} &
  1.77 &
  \multicolumn{1}{l|}{3.20} &
  1.79 &
  0.0845 &
  0.0017 \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Cagtegorised Scenarios\\ \\ {[}3, 0, 0{]}\\ \\ {[}3, 1, 0{]}\\ \\ {[}3, 0, 1{]}\\ \\ {[}3, 1, 1{]}\\ \\ {[}2, 0, 2{]}\\ \\ {[}2, 1, 2{]}\\ \\ {[}1, 0, 2{]}\\ \\ {[}1, 1, 2{]}\\ \\ {[}0.5, 0, 2{]}\\ \\ {[}0.5, 1, 2{]}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.14\\ \\ 0.19\\ \\ 1.66\\ \\ 0.92\\ \\ 0.40\\ \\ 1.36\\ \\ 0.45\\ \\ 3.11\\ \\ 0.43\\ \\ 0.55\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}0.37\\ \\ 0.44\\ \\ 1.28\\ \\ 0.96\\ \\ 0.63\\ \\ 1.16\\ \\ 0.67\\ \\ 1.76\\ \\ 0.66\\ \\ 0.74\end{tabular} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.11\\ \\ 0.25\\ \\ 5.65\\ \\ 1.41\\ \\ 3.83\\ \\ 0.26\\ \\ 0.74\\ \\ 2.90\\ \\ 0.79\\ \\ 0.34\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}0.33\\ \\ 0.50\\ \\ 2.37\\ \\ 1.19\\ \\ 1.95\\ \\ 0.5\\ \\ 0.86\\ \\ 1.70\\ \\ 0.89\\ \\ 0.58\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}0.0022\\ \\ 0.0029\\ \\ 0.0010\\ \\ 0.0008\\ \\ 0.0007\\ \\ 0.0008\\ \\ 0.0008\\ \\ 0.0014\\ \\ 0.0006\\ \\ 0.0010\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}0.0010\\ \\ 0.0014\\ \\ 0.0007\\ \\ 0.0006\\ \\ 0.0006\\ \\ 0.0007\\ \\ 0.0006\\ \\ 0.0008\\ \\ 0.0005\\ \\ 0.0011\end{tabular} \\ \hline
\end{tabular}
\end{table*}

==> Tables/Results2.tex <==
\begin{table*}[t]
\centering
\caption{Results of channel estimation by random forest algorithm.}
\label{tab:RF-Results}
\begin{tabular}{|l|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|l|l|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Random Forest\\ Algorithm for \\ Channel Estimation \\ in LP-IoT Devices\end{tabular}}} & \multicolumn{2}{l|}{\textbf{Training}} & \multicolumn{2}{l|}{\textbf{Testing}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Training\\  time (Secs)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Testing\\  time (Secs)\end{tabular}}} \\ \cline{2-5}
 & \multicolumn{1}{l|}{\textbf{MSE}} & \textbf{RMSE} & \multicolumn{1}{l|}{\textbf{MSE}} & \textbf{RMSE} & & \\ \hline
\textbf{Combined Scenarios} & 3.16 & 1.77 & 3.20 & 1.79 & 0.0845 & 0.0017 \\ \hline
% Add your other rows here, and adjust the line breaks and column types as needed
\end{tabular}
\end{table*}

